DivEMT: Neural Machine Translation Post-Editing Effort Across Typologically Diverse Languages

We introduce DivEMT, the first publicly available post-editing study of Neural Machine Translation (NMT) over a typologically diverse set of target languages. Using a strictly controlled setup, 18 professional translators were instructed to translate or post-edit the same set of English documents into Arabic, Dutch, Italian, Turkish, Ukrainian, and Vietnamese. During the process, their edits, keystrokes, editing times and pauses were recorded, enabling an in-depth, cross-lingual evaluation of NMT quality and post-editing effectiveness. Using this new dataset, we assess the impact of two state-of-the-art NMT systems, Google Translate and the multilingual mBART-50 model, on translation productivity. We find that post-editing is consistently faster than translation from scratch. However, the magnitude of productivity gains varies widely across systems and languages, highlighting major disparities in post-editing effectiveness for languages at different degrees of typological relatedness to English, even when controlling for system architecture and training data size. We publicly release the complete dataset including all collected behavioral data, to foster new research on the translation capabilities of NMT systems for typologically diverse languages.

==> tab_sentence_example.tex <==


S: 47
As soon as you get out of the current, swimming back is no more difficult than normally.

S:54
He referred to the rumors as "political chatter and silliness".

S:93
During blizzards, enough snow to get you stuck can fall in very little time.


%%%%%%
S:12

People may not anticipate that patience and understanding are also necessary for travellers returning home.

MT :  la gente non può anticipare che la pazienza e la comprensione sono  necessari anche per i viaggiatori che tornano a casa.
PE :  la gente non *** immagina   che ** pazienza e ** comprensione siano necessari anche per * chi         fa  ritorno a casa.
EVAL:              D   S              D             D               S                         D S           S   S


MT :  la gente potrebbe non  aspettarsi che la ****** pazienza e la comprensione siano   necessarie   anche   per         i   viaggiatori che tornano     a   casa.
PE :  ** ***** nessuno  però pensa      che la stessa pazienza e ** comprensione debbano essere     [ anche ] riservate @ chi rientra     nel proprio @ [ a ] paese.
EVAL: D  D     S        S    S                 I                 D               S       S                    S           S   S           S   S               S

DUTCH

MT :  mensen verwachten misschien niet ****** dat   geduld en begrip     ook   nodig   zijn voor reizigers die naar huis         terugkeren.
PE :  mensen realiseren zich      niet altijd dat [ geduld en begrip ] [ ook @ nodig ] **** **** reizigers die **** thuiskomen @ hebben.
EVAL:        S          S              I                                               D    D                  D    S            S

MT :  mensen ****** kunnen   niet ** ** verwachten dat geduld en begrip ook nodig zijn voor reizigers die naar huis terugkeren.
PE :  mensen hebben mogelijk niet in de gaten      dat geduld en begrip ook nodig zijn voor reizigers die naar huis terugkeren.
EVAL:        I      S             I  I  S

